Fun-SAT: Functional Corruptibility-Guided SAT-Based Attack on Sequential Logic Encryption

The SAT attack has shown to be efficient against most combinational logic encryption methods. It can be extended to attack sequential logic encryption techniques by leveraging circuit unrolling and model checking methods. However, with no guidance on the number of times that a circuit needs to be unrolled to find the correct key, the attack tends to solve many time-consuming Boolean satisfiability (SAT) and model checking problems, which can significantly hamper its efficiency. In this paper, we introduce Fun-SAT, a functional corruptibility-guided SAT-based attack that can significantly decrease the SAT solving and model checking time of a SAT-based attack on sequential encryption by efficiently estimating the minimum required number of circuit unrollings. Fun-SAT relies on a notion of functional corruptibility for encrypted sequential circuits and its relationship with the required number of circuit unrollings in a SAT-based attack. Numerical results show that Fun-SAT can be, on average, 90x faster than previous attacks against state-of-the-art encryption methods, when both attacks successfully complete before a one-day time-out. Moreover, Fun-SAT completes before the time-out on many more circuits.

==> tables/table1_feature_comp.tex <==
% \begin{table}[]
% \centering
% \caption{Properties of defenses}
% \label{table:feature_comp}
% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
% % \setlength{\extrarowheight}{.75ex}
% \resizebox{0.95\linewidth}{!}{

% \begin{threeparttable}
% \begin{tabular}{@{}l|c|c|c|c|l}
% \toprule
% \textbf{Technique} & \textbf{\begin{tabular}[c]{@{}l@{}}Key \\ sequence\end{tabular}} & \textbf{\# of input} & \textbf{\begin{tabular}[c]{@{}l@{}}Independent \\ key port\end{tabular}} & \textbf{Unroll times} & \textbf{\#DIPS*} \\ \hline

% HARPOON & k               & n           & No                  & $>= k+1$        &  $<10$      \\ \hline
% Comb. Locking & 1               & n           & Yes                  & $>=1$          &  $<2^{\#key bit}$      \\ \hline

% M1      & k               & n           & Yes                  & k            &  $k\times 2^n$       \\ \hline
% M2      & k               & n           & No                   &          &  $2^{k\times n}$       \\ \hline
% M3      & k               & n           & No                   &              &         \\ \bottomrule
% \end{tabular}

% \begin{tablenotes}
%     \item[a] The value for HARPOON is the maximum experimental value from xx tests. The values for M1, M2 and M3 are their theoretical upper bound. The experimental values are close to these bounds. 

% \end{tablenotes}
% \end{threeparttable}}
% \end{table}

==> tables/table2_benchmarks.tex <==
% \begin{table}[]
% \centering
% \caption{Characteristics of benchmarks}
% \label{table:benchmarks}
% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
% % \setlength{\extrarowheight}{.75ex}
% \resizebox{0.95\linewidth}{!}{

% \begin{tabular}{@{}l|c|c|c|c|c|c|c|c|l}
% \toprule
% \textbf{Bench} & s27 & s526 & s1488 & s9234 & s38584 & s15850 & b10 & b12 & b15  \\ \hline
% \textbf{\#PIs} & 4  & 3 & 8 & 19 & 12 & 14 & 11 & 5 & 36  \\ \hline
% \textbf{\#POs} & 1  & 6 & 19 & 22 & 278 & 87 & 6 & 6 & 70  \\ \hline
% \textbf{\#FFs} & 3  & 21 & 6 & 228 & 1452 & 597 & 17 & 121 & 449  \\ \hline
% \textbf{\#Gates} & 120  & 178 & 613 & 1021 & 11748 & 3371 & 214 & 1217 & 8169  \\ \bottomrule

% \end{tabular}}

% \end{table}

==> tables/table3_SATresult.tex <==
% \begin{table*}[]
% \centering
% \caption{Experimental results of UB-SAT attack}
% \label{table:SATresults}
% \setlength{\aboverulesep}{0pt}
% \setlength{\belowrulesep}{0pt}
% % \setlength{\extrarowheight}{.75ex}
% \resizebox{0.95\linewidth}{!}{

% \begin{tabular}{@{}l|c|c|c|c|c|c|c|c|c|c|c|l}
% \toprule
% \textbf{Bench} & \textbf{Key Seq. Len.} & \textbf{\#Unrolling} & \textbf{\#Dips} & \textbf{Runtime} & \textbf{Key Seq. Len.} & \textbf{\#Unrolling} & \textbf{\#Dips} & \textbf{Runtime} & \textbf{Key Seq. Len.} & \textbf{\#Unrolling} & \textbf{\#Dips} & \textbf{Runtime} \\ \hline
% s27            & 1                      & 2                    & 255             &                  & 4                      & 8                    & 65535           &                  & 1                      & 12                   & 255             &                  \\ \hline
% s526           & 1                      & 2                    & 8               &                  & 5                      & 10                   & 32767           &                  & 1                      & 12                   & 8               &                  \\ \hline
% s1488          & 1                      & 2                    & 255             &                  & 2                      & 4                    & 65536           &                  & 1                      & 12                   & 255             &                  \\ \hline
% s9234          & 1                      & 2                    & 524287          &                  & 2                      & 4                    & 2.75e11         &                  & 1                      & 12                   & 524287          &                  \\ \hline
% s38584         & 1                      & 2                    & 4095            &                  & 2                      & 4                    & 1.67e7          &                  & 1                      & 12                   & 4095            &                  \\ \hline
% s15850         & 1                      & 2                    & 16383           &                  & 2                      & 4                    & 2.68e8          &                  & 1                      & 12                   & 16383           &                  \\ \hline
% b10            & 1                      & 2                    & 2047            &                  & 2                      & 4                    & 4194303         &                  & 1                      & 12                   & 2047            &                  \\ \hline
% b12            & 1                      & 2                    & 31              &                  & 2                      & 4                    & 1023            &                  & 1                      & 12                   & 31              &                  \\ \hline
% b15            & 1                      & 2                    & 6.87e10         &                  & 2                      & 4                    & 4.72e21         &                  & 1                      & 12                   & 6.87e10         &                  \\ \bottomrule

% \end{tabular}}

% \end{table*}

